Hybrid Mesh-Gaussian Representation for Efficient Indoor Scene Reconstruction

3D Gaussian splatting (3DGS) has demonstrated exceptional performance in image-based 3D reconstruction and real-time rendering. However, regions with complex textures require numerous Gaussians to capture significant color variations accurately, leading to inefficiencies in rendering speed. To address this challenge, we introduce a hybrid representation for indoor scenes that combines 3DGS with textured meshes. Our approach uses textured meshes to handle texture-rich flat areas, while retaining Gaussians to model intricate geometries. The proposed method begins by pruning and refining the extracted mesh to eliminate geometrically complex regions. We then employ a joint optimization for 3DGS and mesh, incorporating a warm-up strategy and transmittance-aware supervision to balance their contributions seamlessly.Extensive experiments demonstrate that the hybrid representation maintains comparable rendering quality and achieves superior frames per second FPS with fewer Gaussian primitives.

==> sec/1_intro2.tex <==
\section{Introduction}
\label{sec:intro}

Reconstructing high-quality 3D representations from multiple unordered images is pivotal in computer vision and graphics. The neural radiance field (NeRF)~\cite{DBLP:conf/eccv/MildenhallSTBRN20} has recently showcased extraordinary performance by integrating deep learning with volumetric rendering to generate high-fidelity images from novel viewpoints. 
%NeRF optimizes multilayer perceptrons to map spatial coordinates and viewing directions to color and density values, capturing intricate geometry and fine details. Numerous extensions have applied NeRF to video synthesis~\cite{DBLP:conf/cvpr/WenTBT0EFKB23, DBLP:conf/cvpr/ChenWCZLGWW23, DBLP:conf/cvpr/LiSZGL0SLGNL22}, 3D reconstruction~\cite{DBLP:conf/nips/YarivGKL21, DBLP:conf/nips/WangLLTKW21, DBLP:conf/iccv/OechsleP021}, and other areas~\cite{DBLP:conf/cvpr/NaKHHY24, DBLP:conf/cvpr/Li0SPGT24, DBLP:conf/cvpr/0007CS23, DBLP:conf/cvpr/ChenBLBLWP24}. However, NeRF's reliance on dense spatial sampling along rays significantly hampers training and rendering speeds.

3D Gaussian Splatting (3DGS)~\cite{DBLP:conf/eccv/MildenhallSTBRN20} has emerged as an efficient alternative, representing scenes with numerous anisotropic 3D Gaussian primitives that enable real-time, high-fidelity rendering through tile-based sorting and rasterization. By parameterizing scenes as optimized sets of Gaussians from structure-from-motion or random initialization, 3DGS efficiently projects these primitives onto 2D planes to generate images. Subsequent studies~\cite{DBLP:journals/corr/abs-2402-01459, DBLP:journals/corr/abs-2402-04796, DBLP:journals/corr/abs-2406-07499} have utilized 3DGS for accurate reconstructions and mesh extraction to simulate physical interactions. Additionally, 3DGS has been applied to dynamic urban environments for autonomous driving~\cite{DBLP:journals/corr/abs-2401-01339, DBLP:journals/corr/abs-2404-02410, DBLP:conf/cvpr/ZhouLSWS024} and integrated with diffusion models to generate high-quality 3D instances~\cite{DBLP:journals/corr/abs-2402-10259, DBLP:conf/cvpr/LiangYLLXC24, DBLP:conf/cvpr/Chen00L24, DBLP:conf/cvpr/YiFWWX000W24, DBLP:conf/cvpr/Ling00FK24}.

Despite its advantages, 3DGS suffers from excessive redundancy in Gaussian primitives~\cite{DBLP:journals/corr/abs-2406-07499, DBLP:conf/eccv/FangW24, DBLP:journals/pacmcgit/PapantonakisKKLD24}, leading to increased memory usage and slower rendering. Methods such as~\cite{DBLP:journals/corr/abs-2406-07499, DBLP:journals/corr/abs-2311-17245} have focused on pruning redundant Gaussians based on their contributions or significance scores~\cite{DBLP:journals/pacmcgit/PapantonakisKKLD24, DBLP:conf/cvpr/TurkiABPKRZR24}. Techniques like per-pixel error functions, steerable densification~\cite{DBLP:journals/corr/abs-2406-15643}, redundancy scoring, intersection-preserving methods~\cite{DBLP:conf/eccv/FangW24}, and global significance scoring~\cite{DBLP:journals/corr/abs-2311-17245} aim to streamline Gaussian representations. However, these approaches rely solely on Gaussian Splatting, often concentrating primitives in texture-rich and geometrically complex regions, as shown in Fig.~\ref{fig:motivation}.

To mitigate this redundancy, we propose a hybrid GS-mesh representation that integrates textured meshes to handle texture-rich flat areas, thereby reducing the number of necessary Gaussian primitives and accelerating rendering speeds. Textured meshes efficiently express high-frequency information in flat regions, allowing Gaussians to focus on intricate geometries. Specifically, we employ textured meshes with full opacity as backgrounds with specific depth values to minimize Gaussian usage.

Our hybrid approach observes that Gaussians predominantly focus on complex geometries and rich textures. Accurately representing complex geometries typically necessitates detailed meshes, which are often unattainable in real-world captures, leaving Gaussians essential for these regions. Conversely, textured meshes effectively manage flat geometric structures and high-frequency details, significantly reducing Gaussian counts in texture-rich areas. However, extracting ideal meshes from real scenes is challenging due to weak supervision in texture-less areas and difficulties in representing intricate geometries, resulting in geometric errors. To address this, we introduce metrics to prune inaccurate and fine-grained meshes, preventing them from compromising the 3D representation. We then integrate the pruned textured mesh with 3DGS to jointly represent indoor scenes. To further optimize, we employ texture supervision to align mesh-rendered images with ground truth and introduce a transmittance-aware mask to avoid color projection from front objects onto the mesh. As demonstrated in Fig.~\ref{fig:teaser}, our hybrid method significantly reduces Gaussian primitives while maintaining comparable rendering quality to traditional 3DGS.

In summary, our contributions are:
\begin{itemize}
    \item We introduce a hybrid representation combining Gaussian Splatting and textured meshes to effectively reduce Gaussian primitives.
    \item We develop metrics to prune flawed meshes in geometrically complex areas and retain meshes in texture-rich flat regions, facilitating joint rendering.
    \item We propose transmittance-aware supervision for the joint optimization of the hybrid representation, enhancing both rendering efficiency and quality.
\end{itemize}

\begin{figure}[htp]
    \centering
    \includegraphics[width=0.98\linewidth]{Figs/motivation.jpg}
    \caption{Visualization of Gaussian distributions and corresponding rendered images. The hybrid representation significantly reduces the number of Gaussians in texture-rich regions while maintaining Gaussian density in geometrically complex areas.}
    \label{fig:motivation}
\end{figure}

==> sec/2_related2.tex <==
\section{Related Works}
\label{sec:related}

\subsection{3D Gaussian Splatting}
3D Gaussian Splatting (3DGS)~\cite{DBLP:journals/tog/KerblKLD23} has become a significant advancement in novel view synthesis, enabling real-time, high-fidelity rendering. Unlike traditional implicit neural fields that rely on ray marching for volumetric rendering, 3DGS represents scenes with numerous explicit Gaussian primitives rendered through tile-based sorting and rasterization. This explicit representation facilitates faster rendering while maintaining high visual quality.

Subsequent studies have expanded 3DGS's applications across various domains. In human avatar rendering~\cite{DBLP:journals/corr/abs-2402-10483, DBLP:conf/cvpr/LiuZTSZLLL24, DBLP:conf/cvpr/LeeKJ24}, 3DGS enables realistic and real-time avatar animations. In content creation~\cite{DBLP:journals/corr/abs-2404-03575, DBLP:conf/eccv/ZhouFXCCBYWK24, DBLP:conf/cvpr/Ling00FK24, DBLP:conf/cvpr/LuGHCYTZD24}, it allows for efficient generation and manipulation of 3D assets. Additionally, 3DGS has been utilized in scene rendering for autonomous driving~\cite{DBLP:journals/corr/abs-2401-01339, DBLP:journals/corr/abs-2404-02410, DBLP:conf/cvpr/ZhouLSWS024}, offering dynamic and scalable representations of urban environments.

Despite these advancements, 3DGS faces challenges related to the excessive number of Gaussian primitives, which can lead to increased memory usage and slower rendering speeds~\cite{DBLP:journals/corr/abs-2406-07499, DBLP:conf/eccv/FangW24, DBLP:journals/pacmcgit/PapantonakisKKLD24}. Methods such as~\cite{DBLP:journals/corr/abs-2406-07499, DBLP:journals/corr/abs-2311-17245} have focused on pruning redundant Gaussians based on their significance or contribution to the scene representation. Techniques like per-pixel error functions, steerable densification~\cite{DBLP:journals/corr/abs-2406-15643}, redundancy scoring, intersection-preserving methods~\cite{DBLP:conf/eccv/FangW24}, and global significance scoring~\cite{DBLP:journals/corr/abs-2311-17245} aim to streamline Gaussian representations. However, these approaches rely exclusively on Gaussian Splatting, often resulting in a concentration of primitives in texture-rich and geometrically complex regions, as depicted in Fig.~\ref{fig:motivation}.

Our hybrid representation diverges from these methods by integrating textured meshes to handle texture-rich flat areas, thereby reducing the reliance on Gaussian primitives in these regions. This allows Gaussians to focus on accurately representing intricate geometries, optimizing both rendering speed and memory efficiency. Theoretically, our method complements existing Gaussian pruning techniques, offering a perpendicular approach that enhances overall scene representation without solely depending on Gaussian attributes.

\subsection{Hybrid Representation}
To harness the strengths of multiple 3D representations, such as NeRF, meshes, and Gaussian Splatting, various hybrid approaches have been developed~\cite{DBLP:conf/cvpr/Wen0RSW24, DBLP:conf/eccv/DhamoNMSSZP24,DBLP:journals/corr/abs-2408-10041, DBLP:journals/corr/abs-2403-09981, DBLP:conf/cvpr/ZouYGLLCZ24}. These methods aim to combine the detailed geometric modeling of meshes with the expressive rendering capabilities of Gaussian primitives or neural fields.

VMesh~\cite{DBLP:conf/siggrapha/GuoC0HSZ23} represents objects using textured meshes alongside auxiliary sparse volumes to enhance view synthesis efficiency. HybridNeRF~\cite{DBLP:conf/cvpr/TurkiABPKRZR24} merges surface-based and volume-based rendering into a unified model, achieving real-time rendering with high quality. SuGaR~\cite{DBLP:conf/cvpr/GuedonL24} aligns 3D Gaussians with mesh surfaces to facilitate mesh extraction and joint optimization of Gaussians and meshes. GSDF~\cite{DBLP:journals/corr/abs-2403-16964} and NeuSG~\cite{DBLP:journals/corr/abs-2312-00846} enhance surface reconstruction quality by integrating 3DGS with neural Signed Distance Fields (SDF).

MeshGS~\cite{choi2024meshgsadaptivemeshalignedgaussian} introduces regularization techniques to tightly bind Gaussian splats to extracted mesh surfaces, ensuring high-quality rendering. GaMeS~\cite{DBLP:journals/corr/abs-2402-01459} parameterizes each Gaussian primitive using mesh face vertices, enabling mesh-based manipulation of Gaussians. SplattingAvatar~\cite{DBLP:conf/cvpr/ShaoWLWL00024} separates avatar motion and appearance by combining explicit mesh faces with implicit Gaussian-based appearance modeling, facilitating compatibility with animation techniques. GaussianAvatars~\cite{DBLP:conf/cvpr/QianKS0GN24} integrates Gaussian splats onto parametric morphable face models, allowing control over expressions, poses, and viewpoints. HAHA~\cite{DBLP:journals/corr/abs-2404-01053} utilizes Gaussian splatting and textured meshes to efficiently render human avatars with fewer Gaussians, assuming the availability of water-tight SMPL-X meshes and handling object occlusions. Additionally,~\cite{DBLP:journals/corr/abs-2407-16173} combines meshes for room layouts with Gaussian Splatting for other objects using prior segmentation, though it is limited to layouts requiring minimal Gaussians and relies on manually acquired meshes from synthetic datasets, making it less practical for real-world scenes.

In contrast, our method leverages textured meshes to dominate texture-rich areas, effectively reducing Gaussian primitives while maintaining rendering performance similar to traditional 3DGS. By pruning and refining meshes to exclude geometrically complex regions and focusing Gaussians on intricate geometries, our hybrid representation achieves a balance between efficiency and quality that surpasses existing hybrid approaches.
